A Novel Classification Approach for Credit Scoring based on Gaussian Mixture Models

Credit scoring is a rapidly expanding analytical technique used by banks and other financial institutions. Academic studies on credit scoring provide a range of classification techniques used to differentiate between good and bad borrowers. The main contribution of this paper is to introduce a new method for credit scoring based on Gaussian Mixture Models. Our algorithm classifies consumers into groups which are labeled as positive or negative. Labels are estimated according to the probability associated with each class. We apply our model with real world databases from Australia, Japan, and Germany. Numerical results show that not only our model's performance is comparable to others, but also its flexibility avoids over-fitting even in the absence of standard cross validation techniques. The framework developed by this paper can provide a computationally efficient and powerful tool for assessment of consumer default risk in related financial institutions.

==> 01intro2.tex <==
\section{Introduction}\label{sec:intro}

%%%%%%%%%%%%%%%%%%%%%%%%%%GMM
Credit scorecard models have gained considerable attention from both academics and practitioners in the last two decades (\cite{baesens2003benchmarking,lessmann2015benchmarking,brown2012experimental}). This paper investigates the application of Gaussian Mixture Models in credit scoring. A Gaussian Mixture Model (GMM) consists of a finite number of Gaussian variables mixed together with a known weighting scheme (\cite{bishop2006pattern,buckley2008portfolio}). These components with their corresponding means and co-variances can be used to construct clusters from data. Clustering with Gaussian Mixture Models can be thought of as a probabilistic k-means clustering technique with the advantage of considering co-variance in the structure of generated clusters. GMC has been commonly used in a wide range of applications such as data mining, pattern recognition,  as well as signal and image processing, but so far, their application in building scorecard models is missing in the literature.

%%%%%%%%%%%%%%%logistic regression, trees
Some of the simplest classification algorithms for credit scoring include logistic regression, decision trees and discriminant analysis (\cite{hand1997statistical,lee2006mining,zhang2010vertical,yap2011using}). %%%%%%%%%%%%%%%%%%%%%%%%%%SVM
Many of the statistical methods used to construct credit scoring models are focused on conventional methods of comparison. Non-linear or piece-wise linear approaches like the kernel Support Vector Machines with random forrest and data mining approaches, however, have recently gained considerable attention for credit scoring applications (\cite{huang2007credit, bellotti2009support}). These new techniques are shown to make credit scorecards more accurate and efficient. For instance, \cite{ghodselahi2011hybrid} provides a comparative analysis on ten SVM classifiers as the members of the ensemble model and shows the SVM classifier works as well as decision tree classifiers. They also represented a hybrid GA-SVM model by combining genetic algorithms with SVM classifiers. Support Vector Machines are also capable of being a hybrid component with data mining techniques, where clustering and classification stages are done through SVM (\cite{chen2012credit}). Finally, Cluster Support Vector Machine (CSVM) for credit scoring has been reported as an efficient classifier compared to other nonlinear SVM methods (\cite{harris2015credit}).

%%%%%%%%%%%%%%% ANN
Artificial Neural Networks (ANNs) are another type of non-linear machines with clustering and classification layers. They are able to organize unlabeled data according to differences between their characteristics. Various forms of ANNs have been used to build credit scoring models including hybrid neural discriminant techniques and Restricted Boltzman Machines (\cite{lee2002credit,tomczak2015classification}).  \cite{yeh2009comparisons} shows that through different methods of data mining, artificial intelligence outperforms the traditional
discriminant analysis. There are mixed results on efficiency of ANNs for credit scoring, however, as \cite{west2000neural} provides evidence that simple logistic regression outperforms more complicated Neural Networks, such as Multi-layer Perceptron Neural Networks.

%%%%%%%%%%%%%%%%huybrid/combined
In order to improve the accuracy of the credit scoring models, treat data imbalance problems, and eliminate over-fitting, extensive research has been done on development of hybrid and combined methods using various above mentioned machine leaning techniques, including Support Vector Machines (\cite{chen2010combination}), Decision Trees (\cite{chen2010combination,zhang2010vertical}), Fuzzy Classifiers 
with Boosting (\cite{hoffmann2002comparing}), Ensemble Classification techniques (\cite{nanni2009experimental,paleologo2010subagging,xiao2016ensemble}), Neural Networks and Multi-variate Adaptive Regression Splines (\cite{hsieh2005hybrid,lee2005two,hsieh2010data}). Credit Scoring databases often show imbalance data as there are more healthy borrowers in these databases. Accordingly, \cite{han2019gaussian} employs Gaussian Mixture Models for data re-sampling to eliminate imbalance data problem in consumer credit market. In addition, data mining and machine learning techniques can be combined to improve model simplicity, model speed, and model accuracy (\cite{liu2005data, martens2007comprehensible}). Similar to mixed results on the performance of Neural Networks, there are contrasting results on efficiency of combination of multiple classifiers for credit scoring (\cite{tsai2008using,wang2011comparative}).

To conclude our literature overview, it is worthwhile to mention a series of surveys on the subject of credit scoring. First, \cite{baesens2003benchmarking} provides a benchmarking research updated after ten years by \cite{lessmanna2013benchmarking} in which a comparison between 41 classifiers and eight algorithms is studied. Two other examples, \cite{hand1997statistical} and \cite{thomas2000survey} provide reviews on statistical and operational research methods for consumer credit classifications. Last but not least,a very interesting paper by \cite{louzada2016classification} presents an interesting survey of 184 articles in 73 journals in credit scoring, and quite surprisingly Gaussian Mixture Models are not studied in any of them.

%%%%%%%%%%%%%%%%% roadmap
The rest of this paper is structured as follows. In Section~\ref{sec:method}
we first briefly introduce credit features and Gaussian Mixture models, and then present our conceptual GMM-based algorithm, with its clustering, classification and assignment steps, for credit scoring. Section~\ref{sec:emp} gives a comparative analysis of our approach with five other standard models. A managerial guideline and applications of our model for consumer credit risk managers are discussed in Section~\ref{sec:manager}. Concluding remarks in Section~\ref{sec:con} end the paper.

==> tabs/aus_featurs.tex <==
\begin{table}
    \label{ausfeat}
  \centering
  \caption{Australian statistical numerical features}
\begin{tabular}{lcccc}
    \toprule
    Feature & MIN   & MAX   & MEAN  & STD \\
    \midrule
    1     & 13.75     & 80.25     & 31.57  & 11.85 \\
   2     & 0 & 28 & 4.76 & 4.98 \\
   6     & 0     & 28.5    & 2.22  & 3.35 \\
   12    & 0     & 2000     & 184.01  & 172.16 \\
    13    & 1     & 100001    & 1018.39  & 5210.1 \\
    \bottomrule
\end{tabular}
\end{table}




==> tabs/datahead.tex <==
\begin{table}
  \label{datahead}
  \centering
  \caption{Data of German}
\begin{tabular}{lcccccc}
    \toprule
    \textbf{existingchecking} & \textbf{duration} & \textbf{credithistory} & \textbf{purpose} & \textbf{creditamount} & \textbf{savings} & \textbf{employmentsince} \\
    \midrule
    A11   & 6     & A34   & A43   & 1169  & A65   & A75 \\
    A12   & 48    & A32   & A43   & 5951  & A61   & A73 \\
    A14   & 12    & A34   & A46   & 2096  & A61   & A74 \\
    A11   & 42    & A32   & A42   & 7882  & A61   & A74 \\
    A11   & 24    & A33   & A40   & 4870  & A61   & A73 \\
    \toprule
    \textbf{installmentrate} & \textbf{statussex} & \textbf{otherdebtors} & \textbf{residencesince} & \textbf{property} & \textbf{age}   & \textbf{otherinstallmentplans} \\
    \midrule
    4     & A93   & A101  & 4     & A121  & 67    & A143 \\
    2     & A92   & A101  & 2     & A121  & 22    & A143 \\
    2     & A93   & A101  & 3     & A121  & 49    & A143 \\
    2     & A93   & A103  & 4     & A122  & 45    & A143 \\
    3     & A93   & A101  & 4     & A124  & 53    & A143 \\
    \toprule
    \textbf{housing} & \textbf{existingcredits} & \textbf{job}   & \textbf{peopleliable} & \textbf{telephone} & \textbf{foreignworker} & \textbf{classification} \\
    \midrule
    A152  & 2     & A173  & 1     & A192  & A201  & 1 \\
    A152  & 1     & A173  & 1     & A191  & A201  & 2 \\
    A152  & 1     & A172  & 2     & A191  & A201  & 1 \\
    A153  & 1     & A173  & 2     & A191  & A201  & 1 \\
    A153  & 2     & A173  & 2     & A191  & A201  & 2 \\
    \bottomrule
    \end{tabular}%
\end{table}%

==> tabs/japanfeat.tex <==
\begin{table}
    \label{japanfeatu}
  \centering
  \caption{Japan statistical numerical features}
\begin{tabular}{lcccc}
    \toprule
    Feature & MIN   & MAX   & MEAN  & STD \\
    \midrule
    1     & 13.75     & 76.75     & 31.53  & 11.78 \\
   2     & 0 & 28.0 & 4.79 & 4.97 \\
   7     & 0     & 28.5    & 2.22  & 4.98 \\
   13    & 0     & 2000     & 182.01  & 171.55 \\
    14    & 0     & 51100    & 854.34  & 3521.3 \\
    \bottomrule
\end{tabular}
\end{table}




==> tabs/numericalfeatures.tex <==
\begin{table}
\label{tas}
\centering
\caption{Numerical features range of values}\label{tab:tas}
\begin{tabular}{lcccc}
    \toprule
    \textbf{Numerical Variables} & \textbf{MIN} & \textbf{MAX} & \textbf{MEAN}  & \textbf{STD}   \\ 
    \midrule
    duration            & 4   & 72  & 20.90 & 12.06 \\ 
    installmentrate     & 1   & 4   & 2.97  & 1.12  \\ 
    residencesince      & 1   & 4   & 2.84  & 1.10   \\ 
    age                 & 19  & 75  & 35.54 & 11.38 \\ 
    existingcredits     & 1   & 4   & 1.40  & 0.58  \\ 
    peopleliable        & 1   & 2   & 1.15  & 0.36  \\ 
    classification      & 0   & 1   & 0.70  & 0.46  \\ 
    \bottomrule
\end{tabular}
\end{table}

==> tabs/tabComparisonTest.tex <==
\begin{table}
\centering
\caption{Comparison between different models in Testing set of German, Japanese and Australian data.}
\begin{tabular}{lcccccccccccccc}
\toprule
\multirow{4}[5]{*}{Models} & \multicolumn{14}{c}{Testing Results} \\
\cmidrule{2-15}      & \multicolumn{4}{c}{Germany}   & $\qquad$ & \multicolumn{4}{c}{Japan}     & $\qquad$ & \multicolumn{4}{c}{Australia} \\
\cmidrule{2-15}      & ROC AUC  & Precision  & Recall  & F1    & $\qquad$ & ROC AUC  & Precision  & Recall  & F1    & $\qquad$ & ROC AUC  & Precision  & Recall  & F1  \\
      & Score & Score & Score & Score & $\qquad$ & Score & Score & Score & Score & $\qquad$ & Score & Score & Score & Score \\
Linear SVM & 76\%  & 81\%  & 86\%  & 83\%  & $\qquad$ & 92\%  & 77\%  & 89\%  & 83\%  & $\qquad$ & 92\%  & 80\%  & 92\%  & 86\% \\
Logistic Regression & 76\%  & 81\%  & 85\%  & 83\%  & $\qquad$ & 92\%  & 79\%  & 88\%  & 83\%  & $\qquad$ & 92\%  & 82\%  & 84\%  & 83\% \\
Gradient Boosting Classifier & 76\%  & 81\%  & 86\%  & 83\%  & $\qquad$ & 92\%  & 84\%  & 86\%  & 85\%  & $\qquad$ & 93\%  & 85\%  & 78\%  & 81\% \\
Bagging Classifier & 77\%  & 83\%  & 76\%  & 80\%  & $\qquad$ & 92\%  & 85\%  & 89\%  & 87\%  & $\qquad$ & 92\%  & 86\%  & 76\%  & 81\% \\
Random Forest Classifier & 73\%  & 82\%  & 80\%  & 81\%  & $\qquad$ & 92\%  & 89\%  & 80\%  & 84\%  & $\qquad$ & 90\%  & 85\%  & 71\%  & 77\% \\
Guassian Mixture Model & 55\%  & 73\%  & 93\%  & 82\%  & $\qquad$ & 83\%  & 92\%  & 66\%  & 77\%  & $\qquad$ & 93\%  & 78\%  & 90\%  & 84\% \\
\bottomrule
\end{tabular}%
\label{tab:comparison}%
\end{table}%



==> tabs/test_acc.tex <==
\begin{table}
  \centering
  \caption{Add caption}
  \begin{tabular}{lcccccc}
    \toprule
    \textbf{Test set} & \textbf{1}     & \textbf{2}     & \textbf{3}     & \textbf{4}     & \textbf{5}     & \textbf{6} \\
    \midrule
    \#1   & 0     & 226   & 8     & 0     & 8     & 0 \\
    \#0   & 0     & 83    & 7     & 0     & 2     & 0 \\
    Lable & 0     & 1     & 0     & 0     & 0     & 0 \\
    accuracy  &       & 0.73  & 0.47  &       & 0.2   &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> tabs/test_comparison.tex <==
\begin{table}
  \centering
  \caption{Comparison between testing accuracy of different models}
\begin{tabular}{lccc}
    \toprule
    
    Model & \multicolumn{1}{c}{Germany} & \multicolumn{1}{c}{Australia} & \multicolumn{1}{c}{Japan} \\
    \midrule
    LSVM  & 75.15\% & 86.52\% & 84.62\% \\
    \textcolor[rgb]{ .129,  .129,  .129}{LR} & 74.85\% & 84.78\% & 85.52\% \\
    \textcolor[rgb]{ .129,  .129,  .129}{GBCLF} & 74.85\% & 84.35\% & 87.33\% \\
    \textcolor[rgb]{ .129,  .129,  .129}{BCLF} & 71.56\% & 83.91\% & 89.14\% \\
    \textcolor[rgb]{ .129,  .129,  .129}{RF} & 72.46\% & 81.74\% & 87.78\% \\
    GMM   & 70.35\% & 84.78\% & 83.71\% \\
    \bottomrule
    \end{tabular}%
    \label{tab:comparisontest}%
\end{table}%


==> tabs/train_acc.tex <==
\begin{table}
  \centering
  \caption{Add caption}
  \begin{tabular}{lcccccc}
    \toprule
    \textbf{Train set} & \textbf{1}     & \textbf{2}     & \textbf{3}     & \textbf{4}     & \textbf{5}     & \textbf{6} \\
    \midrule
    \#1   & 15    & 402   & 2     & 9     & 19    & 11 \\
    \#0   & 26    & 151   & 203   & 25    & 31    & 22 \\
    ratio \#1 to \#0 & 0.58  & 2.66  & 0.01  & 0.36  & 0.61  & 0.5 \\
    Lable & 0     & 1     & 0     & 0     & 0     & 0 \\
    accuracy  & 0.63  & 0.73  & 0.99  & 0.74  & 0.62  & 0.67 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> tabs/train_comparison.tex <==
\begin{table}
  \centering
  \caption{Comparison between training accuracy of different models}
\begin{tabular}{lccc}
    \toprule
    Model & Germany & Australia & Japan \\
    \midrule
    LSVM  & 85.26\% & 86.09\% & 87.95\% \\
    \textcolor[rgb]{ .129,  .129,  .129}{LR} & 84.83\% & 87.17\% & 88.86\% \\
    \textcolor[rgb]{ .129,  .129,  .129}{GBCLF} & 94.21\% & 98.04\% & 99.32\% \\
    \textcolor[rgb]{ .129,  .129,  .129}{BCLF} & 99.56\% & 98.70\% & 97.73\% \\
    \textcolor[rgb]{ .129,  .129,  .129}{RF} & 99.89\% & 99.35\% & 98.18\% \\
    GMM   & 77.40\% & 83.91\% & 82.27\% \\
    \bottomrule

    \end{tabular}%
    \label{tab:traincompar}%
\end{table}%

